Inducing Constituency Trees through Neural Machine Translation

Latent tree learning(LTL) methods learn to parse sentences using only indirect supervision from a downstream task. Recent advances in latent tree learning have made it possible to recover moderately high quality tree structures by training with language modeling or auto-encoding objectives. In this work, we explore the hypothesis that decoding in machine translation, as a conditional language modeling task, will produce better tree structures since it offers a similar training signal as language modeling, but with more semantic signal. We adapt two existing latent-tree language models--PRPN andON-LSTM--for use in translation. We find that they indeed recover trees that are better in F1 score than those seen in language modeling on WSJ test set, while maintaining strong translation quality. We observe that translation is a better objective than language modeling for inducing trees, marking the first success at latent tree learning using a machine translation objective. Additionally, our findings suggest that, although translation provides better signal for inducing trees than language modeling, translation models can perform well without exploiting the latent tree structure.

==> random_dump.tex <==
 % \textit{Latent tree learning} is the task of grammar induction with the indirect supervision of a downstream task. Recent advances in latent tree learning show that linguistically interesting trees can be induced using unsupervised language modeling or auto-encoding methods while achieving good performance  
  %The earlier works on latent tree learning use natural language inference as the downstream objective to learn the latent constituency parse trees \cite{YogatamaBDGL16,choi2017unsupervised}. 
  %According to \citet{Williams2018a}, the constituency trees induced by such models that use natural language inference as downstream task do not conform to meaningful linguistic structure. However, recent advances in latent tree learning show that linguistically interesting trees can be induced using unsupervised language modeling or auto-encoder-like language modeling objectives while achieving good downstream task performance \citep{shen2018ordered,Drozdov2018DIORA}. In this work, we train two existing latent tree language models \citep{shen2018neural,shen2018ordered} as the decoders of neural machine translation systems to investigate whether machine translation is a good task for latent tree learning. We find that these models discover linguistically plausible trees when trained with the machine translation objective on German-English and Chinese-English data, while achieving translation qualities at least as good as those seen with simple LSTM baseline decoders. Additionally, the trees produced by the machine translation have better average F1 scores with respect to the Stanford parser than those produced by the language model, suggesting that machine translation offers a richer supervision signal for grammar induction than is available from plain language modeling.
  
  
  %Earlier work on latent tree learning uses natural language inference (NLI) as downstream task to learn the constituency trees \citep{YogatamaBDGL16,maillard2017jointly,choi2017unsupervised}. Although these models perform well in the downstream task, \citet{Williams2018a} report that the trees learned by these models are almost completely random, and do not reflect any consistent understanding of sentence structure. However, the recent latent tree learning models reports promising results.
%\citet{shen2018neural} attempt to learn the latent constituency parse trees by using language modeling as downstream task; this model achieves the F1 performance significantly higher than the random tree baseline and sparked interest in latent tree learning with non-NLI objective. \citet{Drozdov2018DIORA} use tree-LSTM based auto-encoding as the downstream tasks and successfully learn the constituency trees are linguistically meaningful. 

%Previous work has shown that incorporating constituency parse information benefits the NLP models. Since it is expensive and time-consuming to annotate the training data, these models obtain the parsed information from parsers which are pretrained on outside treebanks. However, these treebanks are generally small and offer limited domain coverage, and may not be suitable for the kinds of data used in all NLP tasks. This motivates the work on \textit{latent tree learning} which attempts to induce the constituency trees without the direct supervision of annotated parsed data.

%\begin{figure}
%  \centering
%  \includegraphics[width=0.5\textwidth]{length-BLEU.png}
%  \caption{Comparison of sentence level BLEU of the models trained on IWSLT14 (De-En) with BPE tokens for each sentence length buckets. X-asis represents the sentence length baskets and Y-axis represents the sentence level BLEU. PRPN performs competitively with LSTM across the different sentence length baskets. ON-LSTM performs poorly for long sentences. }
%  \label{fig:bleu-length}
%\end{figure}

